ChinaOpen: A Dataset for Open-world Multimodal Learning

This paper introduces ChinaOpen, a dataset sourced from Bilibili, a popular Chinese video-sharing website, for open-world multimodal learning. While the state-of-the-art multimodal learning networks have shown impressive performance in automated video annotation and cross-modal video retrieval, their training and evaluation are primarily conducted on YouTube videos with English text. Their effectiveness on Chinese data remains to be verified. In order to support multimodal learning in the new context, we construct ChinaOpen-50k, a webly annotated training set of 50k Bilibili videos associated with user-generated titles and tags. Both text-based and content-based data cleaning are performed to remove low-quality videos in advance. For a multi-faceted evaluation, we build ChinaOpen-1k, a manually labeled test set of 1k videos. Each test video is accompanied with a manually checked user title and a manually written caption. Besides, each video is manually tagged to describe objects / actions / scenes shown in the visual content. The original user tags are also manually checked. Moreover, with all the Chinese text translated into English, ChinaOpen-1k is also suited for evaluating models trained on English data. In addition to ChinaOpen, we propose Generative Video-to-text Transformer (GVT) for Chinese video captioning. We conduct an extensive evaluation of the state-of-the-art single-task / multi-task models on the new dataset, resulting in a number of novel findings and insights.

==> figure-demo.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=2\columnwidth]{figures/ChinaOpen_0502}
    \caption{Conceptual diagram of the construction of the proposed \emph{ChinaOpen} dataset. Given a set of 100k \emph{Chinese} videos randomly gathered from the Bilibili video-sharing website (Sec. \ref{ssec:data-gather}), we perform automated data cleaning to remove videos either with low-quality annotations or lacking meaningful visual content (Sec. \ref{ssec:data-cleaning}). This leads to \emph{ChinaOpen-50k}, a webly-labeled set of 50k videos for multimodal learning. Moreover, for a multi-faceted evaluation, we build a ground-truthed test set \emph{ChinaOpen-1k} (Sec. \ref{ssec:data-annotation}). Each test video is accompanied with a manually-checked user title, a manually-written content-based caption, manually-checked user tags, and a number of labels describing visual objects / actions / scenes present in the video content. With all the Chinese text translated to English, ChinaOpen-1k is also suited for directly evaluating multimodal models trained on English data. Note that there is no overlap between ChinaOpen-50k and ChinaOpen-1k videos.}
    \label{fig:ChinaOpen}
\end{figure*}
